SParC: Cross-Domain Semantic Parsing in Context

We present SParC, a dataset for cross-domainSemanticParsing inContext that consists of 4,298 coherent question sequences (12k+ individual questions annotated with SQL queries). It is obtained from controlled user interactions with 200 complex databases over 138 domains. We provide an in-depth analysis of SParC and show that it introduces new challenges compared to existing datasets. SParC demonstrates complex contextual dependencies, (2) has greater semantic diversity, and (3) requires generalization to unseen domains due to its cross-domain nature and the unseen databases at test time. We experiment with two state-of-the-art text-to-SQL models adapted to the context-dependent, cross-domain setup. The best model obtains an exact match accuracy of 20.2% over all questions and less than10% over all interaction sequences, indicating that the cross-domain setting and the con-textual phenomena of the dataset present significant challenges for future research. The dataset, baselines, and leaderboard are released at https://yale-lily.github.io/sparc.

==> tables/data_examples.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{p{72mm}}
\Xhline{2\arrayrulewidth}
$D_1$: \newline 
$C_1$: hhhh  \newline 
\\
$Q_1$: \newline 
$S_1$: 
\newline 
$Q_2$: \newline 
$S_2$: \newline
$Q_3$: \newline 
$S_3$: \newline
$Q_4$: \newline 
$S_4$: \newline
\\
$D_2$:  \newline 
$C_2$: hhhh  \newline 
\\
$Q_1$: \newline 
$S_1$: \newline
$Q_2$: \newline 
$S_2$: \newline
$Q_3$: \newline 
$S_3$: \newline
$Q_4$: \newline 
$S_4$: \newline
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{We manually labelled 100 examples into one or more of the above categories. \citet{Bertomeu06} define these thematic relations between questions in database QA dialogues.} 
\label{tb:data_examples}
\end{table}

==> tables/data_semantic.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.78}{
\begin{tabular}{cccccp{75mm}}
\Xhline{2\arrayrulewidth}
Semantic change & Description & \multicolumn{3}{c}{Dataset} & Example\\
   \cline{3-5} && {\scriptsize ConSeq2SQL} 
                & {\scriptsize ATIS} 
                &  {\scriptsize SequentialQA} \\ \hline
Sel & column selection & 20 & 20 & 20 & example\\
Cond & condition & 20 & 20 & 20 & example\\
Group & group by & 20 & 20 & 20 & example\\
Order & order by & 20 & 20 & 20 & example\\
Compare & negate/insert/union & 20 & 20 & 20 & example\\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{We manually partitioned 100 question transfers in several datasets into the above categories. Our dataset consists of large number of answers beyond simple \texttt{SELECT} and \texttt{WHERE}.} 
\label{tb:semantic}
\end{table*}

==> tables/data_turn.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{cccccc}
\Xhline{2\arrayrulewidth}
 & 1 & 2 & 3 & 4 & $\ge 4$\\\hline
\texttt{WHERE}  & 17.1\% & 46.7\% & 54.3\% & 57.1\% & \% \\
\texttt{AGG}    & 26.5\% & 43.1\% & 49.1\% & 53.6\% & \% \\
\texttt{GROUP}  & 8.3\% & 22.8\% & 29.0\% & 31.5\% & \% \\
\texttt{ORDER}  & 6.2\% & 16.3\% & 27.5\% & 32.6\% & \%\\
\texttt{HAVING} & 1.4\% & 4.5\% & 8.0\% & 9.3\% & \%\\
\texttt{JOIN}   & 16.5\% & 38.5\% & 49.8\% & 58.5\% & \%\\
\texttt{Nested} & 1.3\% & 5.6\% & 9.9\% & 11.6\% & \%\\
\texttt{Others} & 9.3\% & 21.8\% & 36.5\% & 44.5\% & \%\\
\texttt{SET}    & 0.4\% & 2.2\% & 7.4\% & 11.1\% & \%\\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{FOR ATIS as well USE PLOTS! We automatically partition the SQL answer of questions in each turn into the above categories. We observe dramatic differences in the types of questions that are asked at each position of the sequence in our dataset.}
\label{tab:data_turn}
\end{table}
